Dissecting Language Models: Machine Unlearning via Selective Pruning

Understanding and shaping the behaviour of Large Language Models (LLMs) is increasingly important as applications become more powerful and more frequently adopted. This paper introduces a machine unlearning method specifically designed for LLMs. We introduce a selective pruning method for LLMs that removes neurons based on their relative importance on a targeted capability compared to overall network performance. This approach is a compute- and data-efficient method for identifying and removing neurons that enable specific behaviours. Our findings reveal that both feed-forward and attention neurons in LLMs are specialized; that is, for specific tasks, certain neurons are more crucial than others. Code from all experiments is available at https://github.com/nickypro/selective-pruning

==> macros.tex <==
% Constants
\newcommand{\R}{\ensuremath{\mathds{R}}}

% Parentheses
\DeclarePairedDelimiter\brac{(}{)}
\DeclarePairedDelimiter\curlybrac{\{}{\}}
\DeclarePairedDelimiter\sqbrac{[}{]}
\DeclarePairedDelimiter\anglebrac{\langle}{\rangle}

% Types
\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\tensor}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\randvar}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\Set}[1]{\ensuremath{\curlybrac*{#1}}}

% Operators
\DeclareMathOperator*{\argmax}{argmax}

% Functions
\DeclareDocumentCommand \softmax {m} {\ensuremath{
    \text{softmax} \brac*{#1}
}}
\DeclareDocumentCommand \sigmoid {m} {\ensuremath{
    \sigma \brac*{#1}
}}
\DeclareDocumentCommand \relu {m} {\ensuremath{
    \text{ReLU} \brac*{#1}
}}
\DeclareDocumentCommand \diag {m} {\ensuremath{
    \text{diag} \brac*{#1}
}}
\newcommand{\indicator}[1]{\ensuremath{\mathds{1}\brac*{#1}}}

% Probability
\DeclareDocumentCommand \Prob {o o m} {\ensuremath{
    P \IfNoValueTF{#1}{}{_{#1}} \IfNoValueTF{#2}{}{^{#2}} \brac*{#3}
}}
\DeclareDocumentCommand \Expect {o o m} {\ensuremath{
    \mathds{E}\IfNoValueTF{#1}{}{_{#1}}\IfNoValueTF{#2}{}{^{#2}}\sqbrac*{#3}
}}
\DeclareDocumentCommand \Var {o o m} {\ensuremath{
    \mathds{V}\IfNoValueTF{#1}{}{_{#1}}\IfNoValueTF{#2}{}{^{#2}}\sqbrac{#3}
}}
\DeclareDocumentCommand \Normal {o m m} {\ensuremath{
    \mathcal{N}\IfNoValueTF{#1}{}{_{#1}}\brac{#2, #3}
}}

% TeX
\newcommand{\citationneeded}{\ensuremath{\texttt{\bf [CITATION~NEEDED] }}}
\renewcommand{\concept}[1]{\py{#1}}



% EFFEX
\newcommand{\effectiveness}{\xi}
\newcommand{\understanding}{\kappa}
\newcommand{\explanation}{\mathbf{o}_B}
\DeclareDocumentCommand \DAU {m} {\ensuremath{
    \text{DAU} \brac*{#1}
}}

